PeFAD: A Parameter-Efficient Federated Framework for Time Series Anomaly Detection

With the proliferation of mobile sensing techniques, huge amounts of time series data are generated and accumulated in various domains, fueling plenty of real-world applications. In this setting, time series anomaly detection is practically important. It endeavors to identify deviant samples from the normal sample distribution in time series. Existing approaches generally assume that all the time series is available at a central location. However, we are witnessing the decentralized collection of time series due to the deployment of various edge devices. To bridge the gap between the decentralized time series data and the centralized anomaly detection algorithms, we propose a Parameter-efficient Federated Anomaly Detection framework named PeFAD with the increasing privacy concerns. PeFAD for the first time employs the pre-trained language model (PLM) as the body of the client's local model, which can benefit from its cross-modality knowledge transfer capability. To reduce the communication overhead and local model adaptation cost, we propose a parameter-efficient federated training module such that clients only need to fine-tune small-scale parameters and transmit them to the server for update. PeFAD utilizes a novel anomaly-driven mask selection strategy to mitigate the impact of neglected anomalies during training. A knowledge distillation operation on a synthetic privacy-preserving dataset that is shared by all the clients is also proposed to address the data heterogeneity issue across clients. We conduct extensive evaluations on four real datasets, where PeFAD outperforms existing state-of-the-art baselines by up to 28.74%.

==> chapter/tables/datasets.tex <==
\begin{table}[!t]
\centering
\caption{Statistics of datasets}
\label{tab:dataset-stats-1}
% \small
\begin{tabular}{lcccc}
\toprule
Datasets  & \# Dimension & \# Train & \# Test & Anomaly (\%) \\
\midrule
SMD  & 38 & 708,405 & 708,405 & 4.16\% \\
PSM  & 25 & 132,481 & 87,841 & 27.76\% \\
SWaT  & 51 & 495,000 & 449,919 & 12.14\% \\
MSL  & 55 & 58,317 & 73,729 & 10.53\% \\
% SMAP & 25 & 135,183 & 427,617 & 12.79\% \\
\bottomrule
\end{tabular}
\end{table}
% Applications & Server & Server & Space & Space 


==> chapter/tables/main_result_2.tex <==
\captionsetup{} %
\begin{table*}[t]
  % \centering
  % F1-score is the harmonic mean of precision and recall.
  % \captionsetup{font=small}
  % textnormal
  \caption{{Quantitative results for various centralized methods on four datasets (Central. represents centralized)}}
  \vspace{-0.3cm}
  % \textbf{\textcolor{red}{Red}}: best in federated setup, All four metrics are expressed in as \%. 
  \label{tab:main_res_centra}
  \resizebox{1\textwidth}{!}{
  % \large
  \renewcommand{\arraystretch}{1.07} % 减小行高
  \begin{tabular}{p{1cm}|c|cccc|cccc|cccc|cccc}
  \toprule
    \multirow{2}{*}{} & \multirow{2}{*}{Methods} & \multicolumn{4}{c|}{SMD} & \multicolumn{4}{c|}{PSM}  & \multicolumn{4}{c|}{SWAT}& \multicolumn{4}{c}{MSL} \\
    \cmidrule(lr){3-6} \cmidrule(lr){7-10} \cmidrule(lr){11-14} \cmidrule(lr){15-18}
  % &  & \small{Precision} & \small{Recall} & \small{AUC} & \small{F1} & \small{Precision} & \small{Recall} & \small{AUC} & \small{F1} & \small{Precision} & \small{Recall} & \small{AUC} & \small{F1} & \small{Precision} & \small{Recall} & \small{AUC} & \small{F1} \\
  &  & {P} & {R} & {AUC} & {F1} & {P} & {R} & {AUC} & {F1} & {P} & {R} & {AUC} & {F1} & {P} & {R} & {AUC} & {F1} \\
    \midrule
    \centering
    % \fontsize{8}{10}\selectfont
    \multirow{8}{*}{{Central.}}
     & {OCSVM} & {4.87} & 23.44 & 49.02 & 8.01 & 24.11 & 69.49 & 31.96 & 35.80 & 77.91 & 64.18 & 19.39 & 70.38 & 19.01 & 19.86 & 52.25 & 19.42 \\
    & {IF} & 9.02 & 39.00 & 32.84 & 14.66 & 24.25 & 52.42 & 42.47 & 33.16 & 75.76 & 62.40 & 18.78 & 68.44 & 9.55 & 58.57 & 41.58 & 16.42 \\
    & {LOF} & 8.19 & 19.72 & 44.93 & 11.58 & 34.27 & 12.35 & 48.38 & 18.15 & 14.01 & 11.54 & 49.12 & 12.66 & 13.06 & 12.92 & 48.37 & 13.25  \\
    % & {Deep-SVDD} & 81 & 61.05 & 80.22 & 69.63 & 97.54 & 39.67 & 69.64 & 56.4 & 50 & 41.76 & 70.88 & 45.51 & 93.03 & 64.6 & 82.02 & 76.25 \\
    & {Autoformer} & 78.45 & 65.10 & 82.16 & 71.15 & 99.94 & 79.06 & 89.52 & 88.28 & 99.90 & 65.55 & 82.77 & 79.16 & 76.93 & 76.50 & 86.90 & 76.71 \\
    & {TimesNet} & 88.00 & 81.44 & 90.48 & 84.59 & 97.32 & 96.62 & \underline{97.76} & 96.97 & 85.50 & 93.69 & 95.75 & \underline{89.41} & 88.78 & 73.61 & 86.26 & 80.48  \\
    & AT & 90.34 & 82.34 & \underline{90.98} & \underline{86.16} & 95.70 & 95.34 & 96.85 & 95.52 & 76.79 & 80.02 & 88.34 & 78.37 & 69.14 & 86.48 & \textbf{90.97} & 76.85  \\
    & {FPT} & 87.60 & 80.79 & 90.15 & 84.06 & 98.36 & 95.82 & 97.60 & \underline{97.07} & 79.80 & 97.04 & \underline{96.09} & 87.58 & 81.10 & 80.35 & {89.07} & \underline{80.72}  \\
    & {PeFAD$_c$} & 87.93 & 94.37 & \textbf{97.00} & \textbf{90.72} & 97.99 & 97.47 & \textbf{98.37} & \textbf{97.72} & 91.19 & 94.91 & \textbf{96.82} & \textbf{93.01} & 80.87 & 82.73 & \underline{90.22} & \textbf{81.79} \\
    %  \midrule
    %  % \fontsize{8}{10}\selectfont
    %  \centering
    % \multirow{6}{*}{{FL}} 
    % & {Autoformer$_{fl}$} & 74.92 & 82.30 &90.74 & 77.23 & 97.77 & 78.88 & 89.12 & 86.64 & 95.04 & 66.68 & 83.26 & 77.59  & 84.09 & 65.57 & 82.42 & 72.66\\
    % & {TimesNet$_{fl}$} & 86.36 & 85.30 & 92.44 & 84.97 & 98.30 & 89.84 & 94.64 & 93.75 & 88.19 & 84.61 & 91.77 & 86.22 & 70.69 & 73.69 & \underline{85.80} & 71.53\\
    % & {AT$_{fl}$} & 87.02 & 83.57 & 91.62 & 84.63 & 97.29 & 80.02 & 89.62 & 87.07 & 49.96 & 41.77 & 70.88 & 45.50 & 81.77 & 69.40 & 83.96 & \underline{73.93}  \\
    % & {FPT$_{fl}$} & 84.93 & 80.08 & 89.85 & 81.49 & 98.56 & 91.78 & \underline{95.66} & \underline{94.92} & 88.07 & 85.66 & \underline{92.28} & \underline{86.74} & 70.90 & 73.25 & 85.52 & 71.85  \\
    % & FedTADBench & 86.01 & 87.02 & \underline{93.32} & \underline{85.77} & 96.57 & 64.41 & 82.20 & 72.36 & 88.73 & 64.93 & 82.28 & 74.50 & 77.69 & 69.37 & 84.09 & 72.26  \\
    % & {PeFAD} & 88.76 & 94.74 & \textbf{97.22} & \textbf{91.34} & 97.93 & 97.46 & \textbf{98.35} & \textbf{97.68} & 87.71 & 89.78 & \textbf{94.43} & \textbf{88.73} & 73.42 & 87.31 & \textbf{92.61} & \textbf{78.94}\\
    % % & {PeFAD} & 88.76 & 94.74 & \textbf{\textcolor{red}{97.22}} & \textbf{\textcolor{red}{91.34}} & 97.93 & 97.46 & \textbf{\textcolor{red}{98.35}} & \textbf{\textcolor{red}{97.68}} & 87.71 & 89.78 & \textbf{\textcolor{red}{94.43}} & \textbf{\textcolor{red}{88.73}} & 73.35 & 87.31 & \textbf{\textcolor{red}{92.54}} & \textbf{\textcolor{red}{78.89}}\\
    % % \midrule
    
    \bottomrule
    \end{tabular}
  }
  \begin{flushleft}
  \footnotesize
        % \ \ \ \ **Anomaly. We replace the joint criterion in Anomaly Transformer~\cite{xu2022anomaly} with reconstruction error for fair comparison.\\
        % \ \ \ \ \ \ (Central. represents centralized)
    \end{flushleft}
\end{table*}


==> chapter/tables/main_results.tex <==
\captionsetup{} %
\begin{table*}[t]
  % \centering
  % F1-score is the harmonic mean of precision and recall.
  % \captionsetup{font=small}
  % textnormal
  \caption{{Quantitative results for various federated methods on four datasets. P, R, and F1 denote Precision, Recall and F1-Score as \% , respectively.}}
  \vspace{-0.3cm}
  % \textbf{\textcolor{red}{Red}}: best in federated setup, All four metrics are expressed in as \%. 
  \label{tab:main_res}
  \resizebox{1\textwidth}{!}{
  % \large
  \renewcommand{\arraystretch}{1.15} % 减小行高
  \begin{tabular}{c|cccc|cccc|cccc|cccc}
  % {p{1cm}|c|cccc|cccc|cccc|cccc}
  
  \toprule
    % \multirow{2}{*}{} & 
    \multirow{2}{*}{Methods} & \multicolumn{4}{c|}{SMD} & \multicolumn{4}{c|}{PSM}  & \multicolumn{4}{c|}{SWaT}& \multicolumn{4}{c}{MSL} \\
    % \cmidrule(lr){3-6} \cmidrule(lr){7-10} \cmidrule(lr){11-14} \cmidrule(lr){15-18}
    \cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13} \cmidrule(lr){14-17}

  % &  & \small{Precision} & \small{Recall} & \small{AUC} & \small{F1} & \small{Precision} & \small{Recall} & \small{AUC} & \small{F1} & \small{Precision} & \small{Recall} & \small{AUC} & \small{F1} & \small{Precision} & \small{Recall} & \small{AUC} & \small{F1} \\
  & {P} & {R} & {AUC} & {F1} & {P} & {R} & {AUC} & {F1} & {P} & {R} & {AUC} & {F1} & {P} & {R} & {AUC} & {F1} \\
    \midrule
    % \centering
    % % \fontsize{8}{10}\selectfont
    % \multirow{8}{*}{{Central.}}
    %  & {OCSVM} & {4.87} & 23.44 & 49.02 & 8.01 & 24.11 & 69.49 & 31.96 & 35.80 & 77.91 & 64.18 & 19.39 & 70.38 & 19.01 & 19.86 & 52.25 & 19.42 \\
    % & {IF} & 9.02 & 39.00 & 32.84 & 14.66 & 24.25 & 52.42 & 42.47 & 33.16 & 75.76 & 62.40 & 18.78 & 68.44 & 9.55 & 58.57 & 41.58 & 16.42 \\
    % & {LOF} & 8.19 & 19.72 & 44.93 & 11.58 & 34.27 & 12.35 & 48.38 & 18.15 & 14.01 & 11.54 & 49.12 & 12.66 & 13.06 & 12.92 & 48.37 & 13.25  \\
    % % & {Deep-SVDD} & 81 & 61.05 & 80.22 & 69.63 & 97.54 & 39.67 & 69.64 & 56.4 & 50 & 41.76 & 70.88 & 45.51 & 93.03 & 64.6 & 82.02 & 76.25 \\
    % & {Autoformer} & 78.45 & 65.10 & 82.16 & 71.15 & 99.94 & 79.06 & 89.52 & 88.28 & 99.90 & 65.55 & 82.77 & 79.16 & 76.93 & 76.50 & 86.90 & 76.71 \\
    % & {TimesNet} & 88.00 & 81.44 & 90.48 & 84.59 & 97.32 & 96.62 & \underline{97.76} & 96.97 & 85.50 & 93.69 & 95.75 & \underline{89.41} & 88.78 & 73.61 & 86.26 & 80.48  \\
    % & AT & 90.34 & 82.34 & \underline{90.98} & \underline{86.16} & 95.70 & 95.34 & 96.85 & 95.52 & 76.79 & 80.02 & 88.34 & 78.37 & 69.14 & 86.48 & \textbf{90.97} & 76.85  \\
    % & {FPT} & 87.60 & 80.79 & 90.15 & 84.06 & 98.36 & 95.82 & 97.60 & \underline{97.07} & 79.80 & 97.04 & \underline{96.09} & 87.58 & 81.10 & 80.35 & {89.07} & \underline{80.72}  \\
    % & {PeFAD$_c$} & 87.93 & 94.37 & \textbf{97.00} & \textbf{90.72} & 97.99 & 97.47 & \textbf{98.37} & \textbf{97.72} & 91.19 & 94.91 & \textbf{96.82} & \textbf{93.01} & 80.87 & 82.73 & \underline{90.22} & \textbf{81.79} \\
    %  \midrule
    %  % \fontsize{8}{10}\selectfont
     \centering
    % \multirow{6}{*}{{FL}} 
    {Autoformer$_{fl}$} & 74.92 & 82.30 &90.74 & 77.23 & 97.77 & 78.88 & 89.12 & 86.64 & 95.04 & 66.68 & 83.26 & 77.59  & 84.09 & 65.57 & 82.42 & 72.66\\
    {TimesNet$_{fl}$} & 86.36 & 85.30 & 92.44 & 84.97 & 98.30 & 89.84 & 94.64 & 93.75 & 88.19 & 84.61 & 91.77 & 86.22 & 70.69 & 73.69 & \underline{85.80} & 71.53\\
    {AT$_{fl}$} & 87.02 & 83.57 & 91.62 & 84.63 & 97.29 & 80.02 & 89.62 & 87.07 & 49.96 & 41.77 & 70.88 & 45.50 & 81.77 & 69.40 & 83.96 & \underline{73.93}  \\
     {FPT$_{fl}$} & 84.93 & 80.08 & 89.85 & 81.49 & 98.56 & 91.78 & \underline{95.66} & \underline{94.92} & 88.07 & 85.66 & \underline{92.28} & \underline{86.74} & 70.90 & 73.25 & 85.52 & 71.85  \\
    FedTADBench & 86.01 & 87.02 & \underline{93.32} & \underline{85.77} & 96.57 & 64.41 & 82.20 & 72.36 & 88.73 & 64.93 & 82.28 & 74.50 & 77.69 & 69.37 & 84.09 & 72.26  \\
    \midrule
     {PeFAD} & 88.77 & 94.74 & \textbf{97.22} & \textbf{91.34} & 97.93 & 97.46 & \textbf{98.35} & \textbf{97.68} & 87.71 & 89.78 & \textbf{94.43} & \textbf{88.73} & 73.42 & 87.31 & \textbf{92.61} & \textbf{78.94}\\
    % & {PeFAD} & 88.76 & 94.74 & \textbf{\textcolor{red}{97.22}} & \textbf{\textcolor{red}{91.34}} & 97.93 & 97.46 & \textbf{\textcolor{red}{98.35}} & \textbf{\textcolor{red}{97.68}} & 87.71 & 89.78 & \textbf{\textcolor{red}{94.43}} & \textbf{\textcolor{red}{88.73}} & 73.35 & 87.31 & \textbf{\textcolor{red}{92.54}} & \textbf{\textcolor{red}{78.89}}\\
    % \midrule
    
    \bottomrule
    \end{tabular}
  }
  \vspace{-0.2cm}
  % \begin{flushleft}
  % \footnotesize
  %       % \ \ \ \ **Anomaly. We replace the joint criterion in Anomaly Transformer~\cite{xu2022anomaly} with reconstruction error for fair comparison.\\
  %       % \ \ \ \ \ \ (Central. represents centralized)
  %   \end{flushleft}
\end{table*}


==> chapter/tables/old_res.tex <==

\captionsetup{} %
\begin{table*}[htbp]
  % \centering
  \caption{Results}
  \label{tab:main_res}
  \resizebox{1\textwidth}{!}{
  \normalsize
  \renewcommand{\arraystretch}{1.1} % 减小行高
  \begin{tabular}{c|cccc|cccc|cccc|cccc|cccccccccc}
  \toprule
    \multirow{2}{*}{Methods} & \multicolumn{4}{c|}{SMD} & \multicolumn{4}{c|}{PSM}  & \multicolumn{4}{c|}{SWAT}& \multicolumn{4}{c|}{MSL} & \multicolumn{4}{c}{SMAP} \\
    \cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13} \cmidrule(lr){14-17} \cmidrule(lr){18-21}
    & P & R & AUC & F1 & P & R & AUC & F1 & P & R & AUC & F1 & P & R & AUC & F1  & P & R & AUC & F1\\
    \midrule
    OCSVM & 4.87 & 23.44 & 49.02 & 8.01 & 24.11 & 69.49 & 31.96 & 35.8 & 77.91 & 64.18 & 19.39 & 70.38 & 19.01 & 19.86 & 52.25 & 19.42 & 18.65 & 72.92 & 62.46 & 29.71 \\
    Isolation Forest & 9.02 & 39 & 32.84 & 14.66 & 24.25 & 52.42 & 42.47 & 33.16 & 75.76 & 62.4 & 18.78 & 68.44 & 9.55 & 58.57 & 41.58 & 16.42 & 17.4 & 88.23 & 57.31 & 29.08 \\
    LOF & 8.19 & 19.72 & 44.93 & 11.58 & 34.27 & 12.35 & 48.38 & 18.15 & 14.01 & 11.54 & 49.12 & 12.66 & 13.06 & 12.92 & 48.37 & 13.25 & 12.97 & 10.14 & 49.92 & 11.38 \\
    Deep-SVDD & 81 & 61.05 & 80.22 & 69.63 & 97.54 & 39.67 & 69.64 & 56.4 & 50 & 41.76 & 70.88 & 45.51 & 93.03 & 64.6 & 82.02 & 76.25 & 47.4 & 57.32 & 73.99 & 51.89 \\
    Autoformer & 78.45 & 65.1 & 82.16 & 71.15 & 99.94 & 79.06 & 89.52 & 88.28 & 99.9 & 65.55 & 82.77 & 79.16 & 76.93 & 76.5 & 86.9 & 76.71 & 81.64 & 57.02 & 77.16 & 67.15 \\
    TimsNet & 88.0 & 81.44 & 90.48 & 84.59 & 97.32 & 96.62 & \underline{97.76} & 96.97 & 85.5 & 93.69 & 95.75 & \underline{89.41} & 88.78 & 73.61 & 86.26 & 80.48 & 94.42 & 53.06 & 76.3 & 67.94 \\
    Anomaly Transformer & 90.34 & 82.34 & \underline{90.98} & \underline{86.16} & 95.7 & 95.34 & 96.85 & 95.52 & 76.79 & 80.02 & 88.34 & 78.37 & 69.14 & 86.48 & \textbf{90.97} & 76.85 & 88.11 & 57.78 & 78.32 & 69.79 \\
    FPT & 87.6 & 80.79 & 90.15 & 84.06 & 98.36 & 95.82 & 97.6 & \underline{97.07} & 79.8 & 97.04 & \underline{96.09} & 87.58 & 81.1 & 80.35 & 89.07 & \underline{80.72} & 89.76 & 53.83 & 76.46 & 67.3 \\
    
     \midrule
    Anomaly Transformer(FL) & 87.02 & 83.57 & 91.62 & 84.63 & 97.29 & 80.02 & 89.62 & 87.07 & 49.96 & 41.77 & 70.88 & 45.5 & 81.77 & 69.4 & 83.96 & 73.93 & 87.81 & 51.51 & 75.27 & 64.93 \\
    TimsNet(FL) & 86.36 & 85.3 & 92.44 & 84.97 & 98.3 & 89.84 & 94.64 & 93.75 & 88.19 & 84.61 & 91.77 & 86.22 & 70.69 & 73.69 & 85.8 & 71.53 & 0.0 & 0.0 & 0.0 & 0.0 \\
    FPT(FL) & 84.93 & 80.08 & 89.85 & 81.49 & 98.56 & 91.78 & 95.66 & 94.92 & 88.07 & 85.66 & 92.28 & 86.74 & 70.9 & 73.25 & 85.52 & 71.85 & 88.29 & 52.71 & 75.87 & 66 \\
    PeFAD & 88.76 & 94.74 & \textbf{\textcolor{red}{97.22}} & \textbf{\textcolor{red}{91.34}} & 97.93 & 97.46 & \textbf{\textcolor{red}{98.35}} & \textbf{\textcolor{red}{97.68}} & 87.71 & 89.78 & \textbf{\textcolor{red}{94.43}} & \textbf{\textcolor{red}{88.73}} & 73.35 & 87.31 & \textbf{\textcolor{red}{92.53}} & \textbf{\textcolor{red}{78.89}} & 92.67 & 53.14 & \textbf{\textcolor{red}{76.28}} & \textbf{\textcolor{red}{67.55}} \\
    PeFAD & 88.76 & 94.74 & \textbf{\textcolor{red}{97.22}} & \textbf{\textcolor{red}{91.34}} & 97.93 & 97.46 & \textbf{\textcolor{red}{98.35}} & \textbf{\textcolor{red}{97.68}} & 87.71 & 89.78 & \textbf{\textcolor{red}{94.43}} & \textbf{\textcolor{red}{88.73}} & 73.35 & 87.31 & \textbf{\textcolor{red}{92.53}} & \textbf{\textcolor{red}{78.89}} & 92.67 & 53.14 & \textbf{\textcolor{red}{76.28}} & \textbf{\textcolor{red}{67.55}} \\
    PeFAD$^*$ & 87.93 & 94.37 & \textbf{97} & \textbf{90.72} & 97.99 & 97.47 & \textbf{98.37} & \textbf{97.72} & 91.19 & 94.91 & \textbf{96.82} & \textbf{93.01} & 87.61 & 75.14 & 86.94 & \textbf{80.9} & 0 & 0 & 0 & 0 \\
    \bottomrule
    \end{tabular}
  }
\end{table*}


==> chapter/tmp.tex <==

% \section{introduction}
% %With the wide application of time-series data in distributed devices, such as financial transactions, industrial production, and medical monitoring, the need for privacy and data security has become increasingly prominent. 
% With the proliferation of sensors and mobile devices, massive volumes of time series data are being collected in a decentralized fashion, enabling various time series applications, %~\cite{hsu2021multiple,taylor2008modelling,cook2019anomaly, rousseeuw2018anomaly, xu2022anomaly, box1970distribution}, 
% such as fault diagnosis~\cite{hsu2021multiple} and fraud detection~\cite{taylor2008modelling,krollner2010financial,mills2008econometric}. A fundamental aspect of these applications is time series anomaly detection
% %Time series anomaly detection is an important and fundamental task in time series analysis
% ~\cite{cook2019anomaly, rousseeuw2018anomaly, xu2022anomaly, box1970distribution}, where the general goal is to find unexpected or unusual observations and/or trends that may indicate errors, frauds, or other
% abnormal situations requiring further investigations, as shown in Figure~\ref{fig:illusion}. % and 

% %Various well-customized models have been proposed to solve this problem, including supervised~\cite{jia2019anomaly,ma2016supervised} and unsupervised~\cite{xu2022anomaly,zhou2023one} methods, which often assume that the models are trained with centralized data collected from edge devices. %Jia et al.~\cite{jia2019anomaly} utilizes a supervised long short-term memory (LSTM) neural network for anomaly detection.
% %Xu et al.~\cite{xu2022anomaly} learned informative time-point associations without using labels. Zhou et al.~\cite{zhou2023one} achieve time series anomaly detection through a reconstruction-based approach.
% % However, most existing methods assume that the models are trained with centralized data collected from edge devices, 

% Due to its significance, substantial research has been devoted to inventing effective time series anomaly detection models~\cite{taylor2008modelling,cook2019anomaly, xu2022anomaly, box1970distribution}, including approaches based on traditional statistics~\cite{li2010urban,liu2008isolation} and neural networks~\cite{wen2019time,kieu2018outlier}. In real-world scenarios, time series (TS) data is often generated at edge devices (e.g., sensors) that are distributed across cities. However, most existing time series anomaly detection models generally assume centralized training data and thus are less effective to handle the decentralized data. Due to the increasing consideration of privacy protection, the data providers may be unwilling to disclose their original TS data, because it is dangerous that a malicious third party can use the real data. With potential efficient processing and lower latencies, decentralized time series anomaly detection becomes a critical issue to enable privacy protection~\cite{mcmahan2017communication} and support existing licensing agreements and data access restrictions~\cite{meng2021cross}.
% % \HAO{Cite Yan Liu's Paper related to federated spatio-temporal modeling (KDD)~\cite{xxx}}.
% %While there has been extensive work on time series anomaly detection, there is a relatively limited amount of work specifically addressing this task within the context of federated learning. 
% % Existing work on time series anomaly detection assumes that the model is trained from centralized data collected from all device.

% %Traditional centralized time series anomaly detection methods perform well in some scenarios, the ensuing problems of data privacy leakage and large computational cost in centralized training become constraints. Therefore, there is a need to incorporate federated learning techniques to achieve effective detection of time series anomaly across multiple device nodes while ensuring data privacy. Thus, we focus on time series anomaly detection under the federated architecture.

% A major challenge in time series anomaly detection is the lack of large amount of data for training. Compared to domains such as Natural Language Processing (NLP) and Computer Vision (CV), datasets for time series anomaly detection are relatively small in scale. It limits further advancements in the field of time series anomaly detection. The pre-trained language model are obtained by training on a large-scale corpus of textual data. 
% % it has achieved great success in the fields of NLP and CV.
% Recently, some works have explored the cross-domain transferability of pre-trained language model, demonstrating it's effectiveness in non-NLP tasks. Drawing inspiration from the success of pre-trained language model in NLP and CV domains, we are motivated to explore it's potential in addressing the challenges of time series anomaly detection within a federated learning framework. 

% In addition, anomalies are usually rare and obtaining labeled data can be exceptionally difficult. Therefore the use of unsupervised learning methods becomes imperative as they eliminates the reliance on pre-labeled data, allowing us to glean insights and patterns from the available time series data. However, typical unsupervised time series anomaly detection often assumes that the training data are all normal points, and the anomalies only appear in the test data. However, there may also be undetected anomalies in the training set, which we call "implicit anomaly". The presence of implicit anomaly can disrupt the model training process. Therefore, we take this factor into full consideration when designing the model. 
% \begin{figure}[htbp]
% 	\centering
% 	\begin{minipage}{1\linewidth}
% 		\centering
% 		\includegraphics[width=0.9\linewidth]{image/intro2.png}
% 		\caption{Illustration of Anomaly detection}
% 		\label{fig:illusion}%
% 	\end{minipage}
% \end{figure}
% % The main idea is as follows. 

% In this work, we propose i) a parameter-efficient federal time series anomaly detection framework based on pre-trained language model, ii) a mask selection strategy based on implicit anomalies and iii) a feature distillation scheme based on privacy protection. 
% The overall architecture consists of one server and multiple clients with local time series data. We adapt pre-trained language model to unsupervised time series anomaly detection. 
% % and deploy them on client side.
% To better capture local information at time points, the client first divided the local time series into non-overlapping patches and employ mask series modeling to analyze the tiem series. 
% By calculating the difference between the reconstructed value and the true value, we can determine whether each time point is an anomaly. 
% % The input of the pre-trained language model is the time series composed of patches that have been partially masked. The output of the model is the reconstructed estimate for each time point, and by calculating the difference between the reconstructed value and the true value, we can determine whether each time point is an anomaly. 
% To address the problem of high communication cost in federated training, we propose a parameter-efficient tuning method, so that the client and the server only need to transfer lightweight parameters to achieve highly accurate anomaly detection.
% Furthermore, we propose a patch mask selection strategy to solve the problem of "implicit anomaly". 
% % Typical unsupervised time series anomaly detection often assumes that the training data are all normal points, and the anomalies only appear in the test data. However, there may also be undetected anomalies in the training set, which we call "implicit anomaly". The presence of implicit anomaly can disrupt the model training process. Therefore, we take this factor into full consideration when selecting masked patches. 
% By giving potential anomalous patches a greater weight to be masked, so as to alleviate the interference of implicit anomalies on training. 
% In addition, we propose a feature distillation scheme to address the problem of inconsistent local training in federated learning. The main idea is to align the learning representation of local and global model on a generated shared data.
% % correct the convergence direction of client and improve the overall training efficiency by aligning

% We performed experiments with \textbf{xx} baselines and 4 datasets, including centralized and federated settings. Compared to all federal baselines, our proposed method, called PeFAD, shows the best detection ability. In addition, our method has surpassed the centralized training methods in many cases. The ablation studies prove that the patch mask strategy and the feature distillation scheme both enhance our method’s capability. 

% Our main contributions are as follows:
% %efficient-tuning results
% \begin{enumerate}
% \item We are the first to introduce pre-trained language model into federated time-series anomaly detection, addressing the challenge of insufficient training data for training in anomaly detection. 
% % By leveraging the cross-domain knowledge transfer capabilities of pre-trained language model obtained through training on large-scale datasets, it is possible to effectively address data scarcity issues in the context of anomaly detection scenarios.

% \item We design a parameter-efficient tuning method for the anomaly detection task under the federated framework. Fine-tuning in the federated framework is typically constrained by computational and communication costs. 
% % By introducing a parameter-efficient fine-tuning approach, we successfully reduce the computational burden on client devices and mitigate communication costs between clients and the server.

% \item We propose a patch mask selection strategy to address "implicit anomaly" during training for unsupervised learning, and design a novel feature distillation scheme that enhances the performance of federal anomaly detection.

% \item We demonstrate that PeFAD achieves optimal performance in time series anomaly detection with modest communication cost, as compared to other federated baselines.
% \end{enumerate}
% % We demonstrate that PeFAD achieves optimal detection performance while ensuring low communication costs, as compared to other federated learning approaches.
% The remainder of this paper is organized as follows. Section~\ref{sec:RELA} reviews related work and analyzes the drawbacks of existing work. Section~\ref{sec:PRELIM} introduces preliminary concepts and the federated time series anomaly detection problem. We then 
%  present our solutions in Section~\ref{sec:METHOD}, followed by the experimental evaluation in Section~\ref{sec:EXPS}. Section~\ref{sec:CONCLU} concludes the paper.
